Shallow Optical Flow Three-Stream CNN for Macro- and Micro-Expression Spotting from Long Videos

Facial expressions vary from the visible to the subtle. In recent years, the analysis of micro-expressions $-$ a natural occurrence resulting from the suppression of one's true emotions, has drawn the attention of researchers with a broad range of potential applications. However, spotting microexpressions in long videos becomes increasingly challenging when intertwined with normal or macro-expressions. In this paper, we propose a shallow optical flow three-stream CNN (SOFTNet) model to predict a score that captures the likelihood of a frame being in an expression interval. By fashioning the spotting task as a regression problem, we introduce pseudo-labeling to facilitate the learning process. We demonstrate the efficacy and efficiency of the proposed approach on the recent MEGC 2020 benchmark, where state-of-the-art performance is achieved on CAS(ME)$^{2}$ with equally promising results on SAMM Long Videos.

==> acknowledgement.tex <==
\vspace{-0.5em}
\section{Acknowledgement}
This work was funded in part by MOHE Grant FRGS/1/2016/ ICT02/MMU/02/2 Malaysia and Shanghai 'The Belt and Road' Young Scholar Exchange Grant (17510740100).
